Correspondence of I- and Q-balls as Non-relativistic Condensates

If a real scalar field is dominated by non-relativistic modes, then it approximately conserves its particle number and obeys an equation that governs a complex scalar field theory with a conserved global U(1) symmetry. From this fact, it is shown that the I-ball (oscillon) can be naturally understood as a projection (e.g., real part) of the non-relativistic Q-ball solution. In particular, we clarify that the stability of the I-ball is guaranteed by the U(1) symmetry in the corresponding complex scalar field theory as long as the non-relativistic condition holds. We also discuss the longevity of I-ball from the perspective of the complex scalar field in terms of U(1) charge violating processes.

==> reply_2.tex <==
Reply to the referee,

We thank the referee very much for reading our manuscript carefully.
We have modified our manuscript as follows.


In the following, we reply the comments in the referee report in order.

*We replace the term ``non-relativistic limit'' to ``non-relativistic configuration'' in the abstract.

*As is mentioned in the Referee report, the non-linearity of the potential plays 
an important role for the existence of the localized solutions.
We added the comment to mention this fact  below Eq. (3.4) as
``Note that owing to the potential shallower than the quadratic one,
a localized solution can exist.''
*Since in the paper, we concentrate on the non-relativistic regime,
 we added the footnote 1;
``In this paper, we concentrate on the simple case of oscillon whose effective potential
is dominated by the quadratic term.''

*If the typical interaction timescale of the background plasma is much faster than 
that of oscillation of $\phi$, the background plasma is expected to be thermalized all time.
Thus, a real time evolution of $\phi$ does not affect the plasma so much.
On the other hand, there are two effects from the background plasma on the dynamics of $\phi$.
One is deformation of the potential (thermal potential) and the other is
the thermal dissipation effect (which is related with noises by FDT).
In the paper, we consider the situation where
the thermal dissipation effects are not effective.
In order to clarify this, we added the following sentence to the footnote 2;
``We assume that the effects of thermal dissipations
are negligible for simplicity, otherwise one has to take them into account.''

*Above section 4.1, we replace ``In the following of this section, we roughly show" 
to ``The following of this section is devoted to show''.

*Above 4.19, we assume a spatially homogeneous background.
It is true that the oscillon configuration is not actually spatially homogeneous.
However, a typical length scale of variations of the amplitude is much longer than
wave length of the produced particle. Thus, assumption of spatially homogeneous
background is supposed to be a good one. We added an explanation about this above 4.19 as
``For produced modes which have momenta compatible with $2\omega$,
the size R and the typical wall width L are rather large.
Thus, the number changing particle production processes which have
typical length scales $\sim1/\omega$ may not be sensitive to the spatial
variations of the amplitude $\partial \ln\Phi/\partial r\sim 1/L\ll \omega$.''
  
 As is mentioned, what we can get from our analysis is not an exact I-ball solution.
 Thus we added the footnote 4:
 `` Strictly speaking, the obtained solution of Eq. (2.12)
 does not exactly satisfy the original equation of motion Eq (2.2).
 In general, there exist fast oscillating corrections $\delta \Phi$ which are found to be small
 in Sec. 4 a posteriori.
 Thus, what one can obtain from Eq. (2.12) is the dominant part of the I-ball solution.''.


--
Kyohei Mukaida, Masahiro Takimoto

